nBIIG: A Neural BI Insights Generation System for Table Reporting

We present nBIIG, a neural Business Intelligence (BI) Insights Generation system. Given a table, our system applies various analyses to create corresponding RDF representations, and then uses a neural model to generate fluent textual insights out of these representations. The generated insights can be used by an analyst, via a human-in-the-loop paradigm, to enhance the task of creating compelling table reports. The underlying generative neural model is trained over large and carefully distilled data, curated from multiple BI domains. Thus, the system can generate faithful and fluent insights over open-domain tables, making it practical and useful.

==> 2_related.tex <==
\begin{figure}[b]
\begin{center}
  \includegraphics[width=0.85\columnwidth]{figures/system_flow.pdf}
 \end{center}
  \caption{System flow.}~\label{fig:system}
\end{figure}

\begin{figure*}[t]
\begin{center}
  \includegraphics[width=\textwidth]{figures/ui_flow.pdf}
 \end{center}
  \caption{\textsc{BIIG} UI.}~\label{fig:UI}
\end{figure*}

\section{Related Work}
\label{related}

Insights generation falls into the wider task of Table-to-text where the goal is to convert structured data into natural language. %, and specifically our work focuses on surface realization part. 
One approach is to use an intermediate step and create a representation of the tabular data, and then use neural model to generate the sentences as done in~\cite{puzikov-gurevych-2018-e2e,elder-etal-2019-designing}. These works mainly use
WebNLG~\cite{webnlg-2017,webnlg-2020}, E2E~\cite{e2e}, and DART~\cite{nan-etal-2021-dart} datasets which use Wikipedia tables, restaurants, or sport data. We follow DART methodology of RDF representation when creating new data for the BI domain.
% Approaches like \textsc{Logic2Text}~\cite{chen2020logic2text} and Logical NLG~\cite{chen2020logical}, use an End-to-end single neural model to decide on the logic and to generate the sentences. Such models suffer from low factuality level, and are still impractical to use in real world scenarios. 

% In~\cite{Zeng_Luo_Huang_Tang_2019} the authors % ns2 they 
% focus on the ranking mechanism and use templates to generate % ns2 create 
% the sentences. \newcite{Shi2021CalliopeAV} focus on visual data story generation and 
% also rely on templates.%-based sentences. % ns2 for creating the sentences.

Many commercial solutions, including Tableau Narrative Science\footnote{\url{tinyurl.com/mr3bnz5n}}, PowerBI\footnote{\url{powerbi.microsoft.com}},  and IBM Congnos Analytics\footnote{\url{www.ibm.com/products/cognos-analytics}}, automatically identify the observations, and then use template-based approach to generate the sentences therefrom. Tools like Arria NLG\footnote{\url{www.arria.com}}, and Automated Insights\footnote{\url{tinyurl.com/yumy7azp}}, on the other hand, are not using templates. Rather, they aim at creating the text from on-the-fly insights definition based on user % ns2 use user 
inputs. The user needs to explicitly specify % ns2 specifies 
the fields that she is interested in, their dimensions, and measures to be covered in the narrative, as well as the analysis (e.g., average, trends).
Based on these inputs the system will generate the sentences using AI-based approach\footnote{From the public available information it is not clear what are the exact technologies used for generation.}. Our approach does not take the user through a % ns2 tedious and 
complicated process of defining the insights. 
In addition, we verbalize  % ns2 and, in addition, it verbalizes 
the sentences in a templateless manner.
 


==> 4_model.tex <==

\section{Methodology}
\label{methods}
\subsection{Table-to-RDF}
\label{sec:RDF-creation}
A data-table comprises a column $X$ of categorical values, and one or more columns $Y_i$ of numerical values. Inspired by existing BI tools, we chose several widespread
% \emph{insight-types} 
types of mathematical operations, aka \emph{types},
that can be readily computed from the table: MAX, MIN, SUM, AVERAGE, VALUE, COMPARE,
% \michal{can we change this to compare?}
% and 
CORRELATED, and 
% in the common case of $X$ consisting of dates (typically years, or months and years), the list also includes 
TREND. 
% In typical BI tools, each such type, or a combination of a few of them, gives rise to an insight. 

Given a data-table, we exhaustively compute all the above mathematical operations
% ns2 - perhaps clarify in the appendix what you mean? specifically, for value, compare, correlated, and trend, its not clear to me what we compute 
% *ns3 - I still think the appendix should explain exactly what we mean by each operation, and how it is being calculated 
% yp dafna will add
over all numerical columns of the table.
% (cf. Appendix \ref{app:insight_calculations}). We denote each such operation along with its result as an \emph{RDF triple}, (or a short sequence thereof) in a style inspired by DART~\cite{nan-etal-2021-dart}.
E.g., for the data-table illustrated in Figure~\ref{fig:process-example}, whose $X$ column consists of years, and $Y$ column % ns2 columns 
is named `Market Cap', with a % ns2 whose 
maximal value $81.2$, occurring in year 2022, we generate the RDF triple
%\begin{center}
$\texttt{[2022, MAX Market cap, 81.2]}$.
%\end{center}

One special RDF triple conveys the title of the case reported. The title provides some context and may be important to explain the meaning, or units, of the table's columns. An example of the format appears in the bottom row of Table~\ref{tab:rdfs}. % ns2 Table~\ref{tab:insight_dist}. 
% The title format RDF triple is:
% \begin{center}
% \texttt{[CONTEXT, TITLE, Worldwide cheese market cap]}
% \end{center}

% E.g., for a table whose $X$ column consists of years, and one of its $Y$ columns is named `Profit', whose maximal value is 36, occurring in year 2018, we generate the following RDF triple:
% \begin{center}
% \texttt{[2018, MAX Profit, 36]}
% \end{center}

The suggested %Each of the suggested % ns2 ultimate 
insights will be generated from a set of one or more % ns2 few 
RDF triples, and will be attributed by \emph{insight type}(s) based on % ns2 being 
the type(s) of the mathematical operations that originated the set of RDF triples.
%More 
Examples can be found in Table~\ref{tab:rdfs}. % ns2 Table~\ref{tab:RDF-example}.
% A single insight, can generally be composed of a single insight-type or a compositions of them.
% In the sequel, we show how we select the ones to be fed into the language model in order to transform them into insights. For now, we just describe them, and their 
% In this work, we chose the intermediate representation of the insights as a list of RDF triples in a style inspired by DART~\cite{nan-etal-2021-dart}, where each item on this list represents a single insight-type.
% \michal{from here to bottom: I think that we can make this shorter by referring to the Figure 1 and Table 1 examples, no? this is what Table 1 is about.. the format..}
% Suppose another measure column is named `Sales', and whose values grow along the years (as we heuristically identify, tolerating small glitches). We express this property as:
% \begin{center}
% \texttt{[2010-2020, TREND\_Sales, UP]}
% \end{center}
% LOWER is an example of a somewhat complex property, where we compare the values of two cells along same column, specifying which is larger.
% E.g., assuming `Profit' in 2012 is 24, lower than in 2018, we express this property over three triplets:
% \begin{center}
% \texttt{[2018, Profit, 36]} \\
% \texttt{[2012, Profit, 24]} \\
% \texttt{[2012, LOWER\_Profit, 2018]}
% \end{center}

The format we use for % ns2 our 
RDF triples is flexible and readily extendable.
% , although, mathematically speaking, is not unlimited in its expressing power.  
It will allow us to expand the list of types 
based on users' demand, % ns2 on demand, as we use our system and see the needs rise, 
while defining RDF triples representation for each new type, and allowing the spread over several RDF triples for more % ns3 move 
involved types. 
% ns2 with individually defined RDF triple representation for each new type,  allowing ourselves to spread over two - three RDF triples in cases of more involved types. 
% \michal{I wonder if we want to discuss this at all.. it can raise questions like Cognos has - for example how to represent more complex insights ,etc...what do you think?} \yotam{I think it is OK this way...}

\subsection{RDF-to-Text dataset}
\label{sec:rdf-to-text_dataset}
Statista\footnote{\url{statista.com}} is an online platform that regularly publishes and updates pages of tabular data on various domains, % ns2 a vast variety of 
% 25 #25 does not sound vast to me 
% ns2 general subjects, 
including economics, sports, demographics, market and opinion research, education, and more. Each webpage $W_i$ in the site comprises a \emph{data-table} $T_i$, a \emph{chart} illustrating the data, 
and, in addition,
a \emph{title} $t_i$, 
the general \emph{subject} $b_i$ of the reported case, and a \emph{summary} $S_i$ of the chart and data-table written by a human expert in the field. 
During December 2021, we crawled $100K$ publicly accessible Statista webpages. Based on these data, 
% ns2 this data, 
we automatically created % ns3 created 
our RDF-to-text dataset, following these steps:
\begin{enumerate}[nosep]
% \item Crawl webpages, from each, extract: data-table $T$ and title $t$ 
% % and general subject $s$
% % , paired with the
% and
% summary $S$ (see \ref{crawl-statista}). 
% % Then, for each downloaded case:
\item Compute all types, denote them as \emph{RDF triples}, $\{r_{ij}\in{R_i}\}$ for each ($T_i$, $t_i$) 
% using Table-to-RDF 
(Sec~\ref{sec:RDF-creation}).
\item Split $S_i$ into sentences $\{s_{ik} \in S_i\}$, and match each sentence % ns2 each 
against a set of  $r_{ij}$s, yielding a 
% n RDF-to-Text 
dataset of pairs of $(s_{ik},\{r_{ij}:M(s_{ik},r_{ij})\})$ with $M$ being the matching function
% $(\{r_{ij} \in R_i\}, \{I_{ik}\in S_i\}$
% thereby announcing the matching sentences
% each mathced sentence
% \emph{insights}, and obtaining an RDF-to-Text dataset consisting of pairs of $(\{\tilde{r} \in \tilde{R}\}, i \in I)$, 
(Sec~\ref{sec:insight_matching}).
\end{enumerate}

% \subsubsection{Crawling Statista}
% \label{crawl-statista}
% During December 2021, we crawled $100K$ publicly accessible Statista webpages, each making a single data point. From each downloaded page, we extracted the data table, title, subject, and summary. \michal{this section seems like repetition of the first step in above.. only adding the number of pages.. maybe we should remove this section, and add the first sentence describing the size etc at the end of the previous section. ?}

% \subsubsection{Candidate Insight Extraction}
% \label{sec:Insight-types} 


% \resizebox{\columnwidth}{!}{
% \small
% \usepackage{hhline}

% \end{table}
% \begin{tabular}{|p{3cm}|p{15cm}|}
%  \hline
%  Insight type  & RDF Triples
%  \\ [0.5ex] 
%  \hline\hline
%  MAX, MIN& \texttt{[[2022, MAX Market cap, 81.2]]} \\ 
%  \hline
%  SUM, AVERAGE & \texttt{[[2000-2020, AVERAGE Market cap, 51.38]]}\\
%  \hline
%  COMPARE & \texttt{[[2022, Market cap, 81.2], [2021, Market cap, 76.1], [2021, COMPARE Market cap, 2022]]} \\
%  \hline
%  TREND & \texttt{[[1960-2022, TREND Market cap, UP]]} \\
%  \hline
%  VALUE & \texttt{[[2022, Profit, 81.2]]} \\
%  \hline
%  CORRELATED &  \texttt{[[Profit, CORRELATED, Market cap]]}\\
%  \hline
% TITLE & \texttt{[[CONTEXT, TITLE, Worldwide cheese market cap]]} \\
%  \hline
%  \end{tabular}

%  \end{tabular}
 
\begin{table}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|} 
\hline
Insight type & RDF Triples \\ 
\hline \hline
MAX, MIN & {[}{[}2022, MAX Market cap, 81.2]] \\ 
\hline
SUM, AVERAGE & {[}{[}2000-2020, AVERAGE Market cap, 51.38]] \\ 
\hline
COMPARE & \begin{tabular}[c]{@{}l@{}}{[}{[}2022, Market cap, 81.2], [2021, Market cap, 76.1], \\{[}2021, COMPARE Market cap, 2022]]\end{tabular} \\ 
\hline
TREND & {[}{[}1960-2022, TREND Market cap, UP]] \\ 
\hline
VALUE & {[}{[}2022, Market cap, 81.2]] \\ % *** ns2 & *ns3 - where did Profit came from?
% yp fixed it here
\hline
CORRELATED & {[}{[}Profit, CORRELATED, Market cap]] \\  % *** ns2 & *ns3 - where did Profit came from?
% yp we need another column to show correlation.
\hline
TITLE & {[}{[}CONTEXT, TITLE, Worldwide cheese market cap]] \\
\hline
\end{tabular}
}
% ns2 
\caption{Examples of RDF representations for supported insights types for the data-table in Figure~\ref{fig:process-example}, for CORRELATED, we assume another column named Profit.}~\label{tab:rdfs}
% ns2 
% \caption{Examples of RDF representations for supported insights types for the data-table appears in Figure~\ref{fig:process-example}.}
\end{table}


\subsubsection{RDF $\leftrightarrow$ Insight Matching}
\label{sec:insight_matching}
\looseness=-1
Given a data-table and title ($T_i, t_i)$ from which a set of RDF triples $\{r_{ij} \in R_i\}$ are generated, and given the corresponding summary $S_i$ split into sentences $s_{ik}$, we seek to match, using rule-based heuristics, a subset of $R_i$ to each sentence $s_{ik}$ in $S_i$.
% To achieve this,
% Now, having generated the set of candidate triplets $\tilde{R}$ (Sec. \ref{sec:RDF-creation}), 
% we 
% split $S_i$ into sentences $s_{ik}$s, and 
% use rule-based heuristics to tell which $s_{ik}$ matches which set of $r_{ij}$s. 
Sentence $s_{ik}$ is said to match an RDF triple $r_{ij}$, denoted  $M(s_{ik},r_{ij})=True$, if it contains 
% ns2 - pls verify
(1) the data-table cell value and its associated column or row names, as mentioned in 
$r_{ij}$, % ns3 the triple, 
or a strongly related alternative (like rounding of the cell value, or plural/singular inflection of a column/row name); 
% ns2 (1) the data-table cell and its coordinates (column/row names) mentioned in the triple, or a commonly verbalized alternative thereof (like number approximation, or plural/singular inflection) 
and (2) any word associated by a pre-defined dictionary with the type specified in 
$r_{ij}$. % ns3 the triple. % ns2 triple. 
For example, 
the pre-defined dictionary for MAX includes % ns2 TREND is associated by this dictionary with 
words like: ``highest'', ``largest'', ``peaked'', ``leading'', etc. % ns2 ``trend'' etc.
%\michal{consider here an example}
Note that a given $s_{ik}$ may match zero, one, or more $r_{ij}$s.
Each statista instance $W_i$ is thus associated with a set of pairs  $\{(s_{ik},\{r_{ij}:M(s_{ik},r_{ij})\})\}$. 
We manually evaluated the matching quality over 100 randomly selected examples. In more than 87\% of the cases %the vast majority of the cases, 
the triples conveyed information fully consistent with the contents of the sentence. 
In total, we identified $59K$ 
sentence/triple(s) matching % ns3 matching 
pairs, % ns2 match $59K$ such pairs, 
split according to $0.9/0.1/0.1$ to train % ns2 train 
/ test / validation sets, with $53K/3K/3K$ pairs, % ns3 examples, 
respectively. 
% ns2 val sets with $53K/3K/3K$ examples.
% *** ns2 - if time permits, add an analysis saying that we manually examined a random sample of 50 matches and concluded most (all?) are fine, and provide a table with ~3 examples?
% \michal{I think we should add here a sentence of how many samples we have after this step.}
% we mark that sentence as an insight and add a pair of 
% that matches the triplet set, and we add a pair of  $(triplet\textrm{-}set, insight)$
% \begin{center}
% $(triplet\textrm{-}set, insight)$
% \end{center}

%Apart from splitting and varifying that the insight is indeed valid, inspired by industry practices\footnote{\url{docs.microsoft.com/en-us/power-bi/consumer/end-user-insight-types}} and academic works~\cite{chen2020logical,perlitzDiversity2022} attach a specific type for each candidate insight, we use 
% a list of $6$ supported types including: superlative (max, min), aggregation (average, sum), comparison, trend (for time-series data), value/most recent (for time-series data), and correlation. 
%the same list of types described in the section \ref{sec:RDF-creation}.
%For each type we compiled a dictionary of English words that may indicate the type and used it to detect relevant sentences. For example, for insight type ``trend'' we look for terms like: ``peak'',``grew'', ``decline'', ``decrease'', ``drop'', etc. 
% To evaluate the quality of type extraction, we randomly extracted $200$ sentences and their assigned types and asked 3 experts to verify the types. The quality was $91\%$. 
% In total, we extracted around $1.5$ candidates of insights per each of the $100K$ data-tables, thereby obtaining a dataset of $150K$ (data-table, title, subject, candidate insight). 
% each is associated with at least one type. For example, this sentence ``In 2022, the growth of China's tourism industry contribution to GDP amounted to 59.9 percent, down from 9.3 percent in the previous year.'' includes both \textit{most recent} and \textit{comparison types}.
% In parallel, we calculate per table all the relevant types. 
% of each such identified insight.
% We identified several types of insights, according to the type of information they convey about the data table. This is an initial list, that can be readily expanded.
% With each type $t$, we associate (1) a computation of a value over the \emph{data table}, or a verification of a numerical property, and (2) a list of English words whose inclusion in a sentence may indicate that the sentence conveys an information of type $t$.

% Given a Statista webpage, we compute, for each measure column $Y$ in the \emph{data table}, the features associated with each type $t$ above. Then, we go over the sentences of the \emph{summary}, looking for a sentence that contains the feature (i.e., a cell value and coordinates, or a commonly verbalized alternative thereof; e.g., for the above triplet, the sentence is to contain both 2018 and 7.2), and any of the dictionary words associated with $t$ ('peak', 'highest', etc. in our example).
% Note that a given sentence may satisfy the feature triplet and the dictionary words of more than one type.
% Once the correctness of the candidate is verified, we add a pair of (\textit{tripletset}, sentence) to the training data.
% The tripletset contains all the RDF triplets expressing computed features that matched to this sentence, along with the title triplet. For example, \{\texttt{[[‘51.38’, ‘Market cap’, ’AVERAGE’],[CONTEXT, TITLE, ``Worldwide cheese market cap 1960-2020'']]},``The average worldwide cheese market cap across the years 1960-2020 is 51.38''\}.

% Each candidate insight $\tilde{I}$ extracted in \ref{sec:Insight-types}, includes some information, namely: \textcolor{blue}{type(s)} associated to it, \textcolor{orange}{numeric value(s)} (textual or numeric) and some \textcolor{mygreen}{column/row name(s)}. Once we extract these from the $\tilde{I}$, we check whether this information is aligned with each of the corresponding $\tilde{R}$ For example, for the given table in Figure~\ref{fig:RDF-example} and a sentence ``The \textcolor{blue}{average} number of cheese \textcolor{mygreen}{market cap} across the years \textcolor{mygreen}{1960-2020} is \textcolor{mygreen}{51.38}'', we need to verify that the average of the the market cap column is indeed around 51 and that those year range is covered by the table. \yotam{}
% In addition to using this set for generation training, we also use the training set of our data to learn the frequency distribution over groups of triplets.
%, as they are grouped together into a set paired with one insight. %Note that a given sentence may satisfy more than one type.

% \michal{I think this section should be discussed before in 4.1}
% Table~\ref{tab:RDF-example} shows the corresponding examples of the supported insights, and their RDF representation. For example, \texttt{[2022, MAX\_Market cap, 81.2]} expresses the fact that along the measure column named ``Market cap'', the maximum value is $81.2$, and it is obtained in $2022$. The context reflecting the title is captured by \texttt{[CONTEXT, TITLE, ``Worldwide cheese market cap'']}. 

% \dafna{we now use slightly different formatting of the RDFs, and we decided to ignore the 'types' that Yotam defined. shall we remove these types from here?} 
% % how are we extracting the RDF triplets from a table.
% % explain how we get ALL the triples.
% \dafna{expand here}
% \yotam{make sure you enumerate the types here: "superlative (max, min), aggregation (average, sum), comparison, trend (for time-series data), value/most recent (for time-series data), and correlation." as I am referring the reader to this section.}

\begin{figure}
\begin{center}
  \includegraphics[width=1\columnwidth]{figures/trainset_type_dist.pdf}
 \end{center}
 % ns3 - rewrote the caption
 \caption{\textbf{Training set type distribution}: In blue we see the distribution for the data created via RDF $\leftrightarrow$ Insight matching. In orange we see the number of -- potentially noisy -- examples added through augmentation. Not observable %in the figure 
  are the un-augmented counts for SUM and AVERAGE which are $2$ and $39$, respectively.}~\label{tab:insight_dist}
  % ns3 \caption{\textbf{Training set type distribution}: Blue are examples from the labeled dataset, orange are noisy labels for the classes that are absent from the training set. Not observable %in the figure are the un-augmented counts for SUM and AVERAGE which are 2 and 39, respectively.}~\label{tab:insight_dist}
\end{figure}

\begin{table*}[t]
\label{tab:rdf2text_eval}
\centering
\small
% \resizebox{\textwidth}{!}{

\begin{tabular}{lc|cccccc}
Model      & Params & BLEU~$\uparrow$ & METEOR~$\uparrow$ & TER~$\downarrow$ & chrF++~$\uparrow$ & PARENT $\uparrow$ & BLEURT~$\uparrow$  \\ 
\hline
t5-small   & 60M    & 40.18           & 0.58              & 56.69            & 59.34             & 0.36              & 0.27               \\
t5-base    & 220M   & 47.73           & 0.64              & 50.15            & 64.60             & 0.43              & 0.35               \\
bart-base  & 140M   & 49.54           & 0.65              & 48.50            & 65.60             & 0.44              & 0.35               \\
bart-large & 400M   & 49.98           & 0.65              & 49.39            & 66.13             & 0.44              & 0.35               \\
t5-large   & 770M   & \textbf{51.52}  & \textbf{0.67}     & \textbf{47.28}   & \textbf{67.21}    & \textbf{0.46}     & \textbf{0.39}            

\end{tabular}
% }
\caption{\textbf{Test set evaluation results:} Evaluation % ns3 Extensive evaluation 
on multiple metrics shows that capacity is a useful indicator for performance under all measured metrics.}\label{tab:rdf2text_eval}

\end{table*}

\subsubsection{Augmentation}
\label{sec:augmentation}
Our initial training set type distribution, as illustrated in Figure~\ref{tab:insight_dist} is showing a clear bias towards the simpler non aggregate types (e.g., VALUE), leaving very few examples for other types (e.g. SUM, AVERAGE).
% \michal{why we need this referring sentence?} 
% As described later in Section \ref{human_eval} 
The scarcity of training examples prevents the model from properly generating 
coherent % ns3 semantically consistent 
texts for these types. 
% ns3 types, a %major
% priority for our system.
To address that, % ns3 As a remedy, 
% To circumvent this difficulty, 
we propose to augment the 
RDF $\leftrightarrow$ Insight matching train data, % ns3 labeled training dataset 
with additional weak % ns3 noisy 
labeled data, comprising of RDF triples gathered from the training set tables and corresponding %text 
weak % ns3 noisy 
labels generated by a Large Language Model (LLM).
Specifically, we generated RDF triples corresponding to the SUM and AVERAGE types that 
appear only % ns3 appear 
$2$ and $39$ times, respectively, % ns3 respectfully, 
in the original training dataset. 
This was done through the following steps: % ns3 Gathering the data amounted to:
\begin{enumerate}[nosep]
\item Extract RDF triples from 500 ($T_i$, $t_i$) pairs.
% (Sec~\ref{sec:RDF-creation}).
\item Group single type RDF triples to include TITLE and SUM/AVERAGE.
\item Generate weak % ns3 noisy 
labels via few-shot learning with a \textit{GPT-J-6B} (Sec~\ref{GPT-J}).
\end{enumerate}

\subsubsection{Few-shot Learning with GPT-J-6B}
\label{GPT-J}
\textit{GPT-J-6B}~\cite{gpt-j}, is a 6B %billion 
parameter, autoregressive text generation model trained on \textit{The Pile} \cite{gao2020pile}. We chose this model as our weak % ns3 noisy 
labeler since these types of LLM have proven to perform well as in context learners \cite{brown2020language} but are unfeasible for deployment in most applications. For each unlabeled example, 
we used a prompt with $5$ (RDF triples, text insight) pairs as context,
% ns3 inputted a prompt that contained 5 (RDF triples, text insight) examples as context,
%an example of such input can be found , 
followed by % ns3 and 
an RDF triple we wish to label (see Figure~\ref{fig:few-shot} in the Appendix). Given this model input, the generated sequence was then taken as the weak % ns3 noisy 
label.

\subsection{RDF-to-Text Model}
\label{genenration}
\looseness=-1Aiming for relative % ns3 maximal 
simplicity and flexibility we followed~\cite{harkous2020have} and chose to frame RDF-to-Text as a sequence-to-sequence problem. To prevent information loss attributed to the structure of the triple set we encode this structure into the linearized representation by replacing the \texttt{","} separators appearing inside and between triples with \texttt{[W]} and \texttt{[B]} tokens, respectively, 
that % ns3 these 
were then were defined as new special tokens for the model to learn during training. % ns3 learn.
We % ns3 we 
used two Pre-trained Language model families, T5~\cite{raffel2020exploring} and BART~\cite{lewis2019bart} which are based on the Transformer \textit{encoder-decoder} % ns3 \textit{encoder-decider}
architecture~\cite{vaswani2017attention}. % and mostly differ in their pre-training corpus and pre-training scheme.
Following~\cite{ribeiro2020investigating}, we %specifically
experimented with \textit{t5-small} / \textit{t5-base} / \textit{t5-large} %(60M / 220M / 770M parameters) 
and \textit{bart-base} / \textit{bart-large}. %(140M / 400M parameters).
Models were trained on our newly generated datasets (augmented and unaugmented) from Section \ref{sec:rdf-to-text_dataset}, Implementation details can be found in Appendix \ref{A: Implementation details}.

\subsubsection{RDF-to-Text Evaluation}
We use a wide range of automatic metrics to evaluate the 
quality of the generated text. % ns3 text generation quality.
We report the official WebNLG~\cite{webnlg-2017} evaluation metrics 
BLEU~\cite{papineni2002bleu}, % ns3 BELU~\cite{papineni2002bleu}, 
METEOR~\cite{banarjee2005meteor}, and TER~\cite{snover-etal-2006-ter}, along with chrF++~\cite{popovic-2017-chrf}, a character n-gram based metric.
Since the above n-gram % ns3 n-grame 
based metrics are limited in their capacity to consider the semantic meaning of words \cite{novikova-etal-2017-need}, we also report %additionally report other 
metrics % ns3 on metrics that were 
suggested by DART~\cite{nan-etal-2021-dart}, such as BLEURT~\cite{bleurt}, that had been shown to 
perform well % ns3 be a top performer 
along the learned semantic similarity metrics. 
To further % ns3 also 
account for generation consistency between the RDF triple and the generated text, % ns3 text, 
we also include PARENT~\cite{dhingra2019parent}, which aligns reference, generated text and 
triple(s) % ns3 triplet 
n-grams. Table \ref{tab:rdf2text_eval} presents the automatic evaluation % ns3 evaluation 
scores on the test set for models in a range of capacities trained on the augmented dataset. 
% ns3
As expected, as the language model size increases, the evaluation scores are typically improved across all metrics, especially for the t5 models, with t5-large obtaining the best performance. % ns3 
% Results indicate that capacity is a useful indicator for performance under all measured metrics.


\subsection{RDF-triples Recommendation}
\label{sec:ranking}
\looseness=-1
%In the following section 
Next, we describe two methods used for recommending which of the 
candidate RDF-triples % ns3 multiple candidate RDF-triple 
generated using our Table-to-RDF methodology will be converted to text and eventually presented to the user.

\subsubsection{Na\"ive Recommendation}
\looseness=-1
This approach provides the user with all 
potential % ns3 relevant // if its naive, I assume it can not pick the 'relevant' insights
insights for a given data-table, each verbalized into a standalone sentence. This enables the user with a straightforward way to select % ns3 an easy and flexible way to work with 
insights she is interested in. 
% As this method does not require any prior knowledge about the user, it will be the first to be used, once the user interacts with the system, his preference will be registered and recommenations can be done according the the user preference.
\subsubsection{Subject-aware Recommendation}
\looseness=-1
A direct outcome of our training data is an associated distribution of the RDF types matched to 
manually written % ns3 gold 
insights, i.e., the \emph{prior}. 
Specifically, we segmented our training % ns3 the 
data into groups using $3$ verticals: time-series (y/n), multi-column (y/n), and subject (list of $25$), giving rise to a % ns3 a 
total of $100$ segments. For each segment, we 
evaluated the type distribution our data. % ns3 collected a distribution of sets of types. 
% \emph{propertie}.
%its insights types. 
% ns3
This analysis suggests which types are more common in each segment, based on our automatic analysis of the Statista data.
% ns3 
% segmentation allows us a finer-granularity view of what experts in the field found interesting in each segment. 
% ns3
Correspondingly, given the segment of a data-table being considered, we sample $4-6$ types from the estimated prior distribution of that segment. 
% ns3
% Given that a data-table belongs to some segment, we will sample by this prior 
%from its distribution 
% between 4-6 sets of types. 
%insights.
% We randomly select a group $G$ of types, according to the prior learned in the training stage. 
We then realize each type as a triple, by computing the associated % ns3 implied 
measure (e.g, MAX, MIN) over a $Y$ column.
% aligning coordinates in case of multiple triples in the set. % *ns3 - not sure what this means, can you try to clarify?
% yp removed this line
When more than one candidate triple can fit a requested type, % ns3 fit, 
we select the most extreme one % ns3 `extreme' 
(e.g., largest maximum, or smallest minimum). 
% The generated triple set is finally fed into the language model which generates an insight therefrom. 

% With our training data, we associate the histogram of the different sets of \emph{properties}. Namely, each matching pair $(triplet\textrm{-}set, insight)$ in the training data contributes 1 to the occurrence count of the set of properties corresponding to the triplet-set. We thus learn the typical distribution of the properties. We further split these histograms by whether $X$ is date or not, whether the table contains multiple measure columns or not, and the \emph{subject}, thus yielding a \emph{prior} that maps from (is-X-date, is-Y-multiple, subject) to (relative) frequencies of the properties of the triplet-sets.
% In Sec. \ref{sec:ranking} we use this \emph{prior} as one of the optional drivers for the recommendation of which candidate triplets are to be fed into the language model for verbalization into an insights.


==> 5_evaluation.tex <==


\section{Human Evaluation}
\label{human_eval}

\subsection{Quality of Generated Insights}
\looseness=-1
To measure the overall quality of our system, we conducted an evaluation % ns3 a thorough evaluation 
with three NLP experts. We sampled $66$ tables from the test set, 
% ns3
and automatically generated insights for each table using the {\it t5-large\/} model, ending up with $529$ insights.
% ns3 and had our system, in its full-stack, and using our largest RDF-to-Text model (\textit{t5-large}), generates insights for them. Our system generated a total of $529$ insights. 
Each insight was evaluated w.r.t faithfulness and fluency, and % ns3 type consistency (
whether its type was consistent with the recommended type. % ns3 ). 
% ns3
As depicted in Table~\ref{tab:human-eval},
% ns3 Table~\ref{tab:human-eval} summarizes the results and shows that, 
on average $90\%$ of the insights were consistent with their type, $93\%$ were marked as fluent adn $88\%$ 
were found to be factualy consistent with the data-table. % ns3 showed a strong factual consistency with the table, 
These factuallity scores are distinctively higher than those obtained when using End-to-end methods \cite{chen2020logical} or other training datasets  \cite{nan-etal-2021-dart} with factuallity scores lower than $50\%$ and $60\%$ respectively. 
% ns3 very fluent. // not sure what 'very' means here since we do not elaborate what we asked the experts
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|ccccccc||c}
\hline
 & \multicolumn{7}{c||}{Insight Type}&\\
    \cline{2-8}
 \hline
&MIN &  MAX & SUM & AVG. & COMP. & TREND & VAL.& AVG\\ \hline
Factuality & 0.88  & 0.98  & 0.92  & 0.91  & 0.84  & 0.78  & 0.81& 0.88 \\ 
Consistency & 0.85  & 0.93  & 0.93  & 0.90  & 0.92  & 0.90  & 0.86 & 0.90\\ 
Fluency & 0.98 & 0.98 & 0.92 &0.82 & 0.95 & 0.9 & 0.97& 0.93\\
\hline
\end{tabular}
}
% ns3
\caption{Insights quality based on manual evaluation. 
% ns3 \caption{Insights quality for the augmented model. 
}
\label{tab:human-eval}
\end{table} 

To quantify the impact of training set augmentation (see Section \ref{sec:augmentation}), 
we repeated the evaluation with % ns3 we applied the same evaluation described above to 
the model trained with the un-augmented data. % ns3 training set. 
As expected, in the augmented model, SUM and AVERAGE show significant factuality improvement of $49\%$ and $42\%$, respectively. No major differences are noted for the other types (see Figure~\ref{fig:aug_vs_unaug} in the Appendix). 

\subsubsection{Error Analysis}
% *ns3 - add opening - e.g., We performed manual error analysis over xx examples selected at random. 
% yp ok
We performed manual error analysis over insights that labelled as non factual in the human evaluation task above.
% ns3
Our training guides the model to only use numbers included in the input. Correspondingly, we observe almost no number-related errors. 
% We carefully trained the language model to use numbers it sees in the input and only them. This bore fruits in almost no number-related errors. 
A few remaining factuality issues are: % ns3 are 
(\RomanNumeralCaps{1}) The % ns3 the 
model might add explanations by % ns3 from 
its own (e.g., \textit{In 2020, 20283 illegal immigrants used the Eastern Mediterranean route to reach the European Union through the Canary Islands.} The input did not contain any Canary Islands on the route from Eastern Mediterranean to Europe).
(\RomanNumeralCaps{2}) In case of multi-column table, the direction of the operation (e.g., maximum over a row or over a column) might show wrong in the sentence. 
(\RomanNumeralCaps{3}) Since the model learns to use the title as annotation of the data numbers (what they count and which units), 
a complex title might yield inaccuracies. % ns3 sophisticated title, that contains an overall impression from the data, might bring about inaccuracy. 
E.g., for a case titled \textit{Growth in health care expenditures in Poland 2014-2020} 
% ns3 that presents yearly health care actual expenditures in Poland (that indeed grow along the years),
one generated insight is \textit{The average annual growth in health care expenditures in Poland during the observed period was 631 percent.} which is inaccurate, as the average is computed over the actual expenditures, not their growth.
% We carefully trained the language model to use numbers it sees in the input and only them. This bore fruits in almost no number-related errors. Very rarely a number shows in the generated insight that we can not tell its source. The same goes for two or more numbers and the size relation between them. Extra words, however, do show here and there, as if the model adds explanations from its own.  
% A source of non-fluent, or at times, even awkward, text results are the titles, which the model learned to use as annotation, or illustration of the numbers (what they count and which units). When a sophisticated title, that consists also of an overall impression from the data, plays the role of unit annotation in the sentence, the sentence becomes non-fluent and cumbersome.  In case of a multi column table, the direction of the operation (e.g., maximum over a row or over a column) might show wrong in the sentence (rarely, but happens). 
% \dafna{add somewhere, perhaps in the future work? that there is room for improvement in both: the intermediate representation, and the language models}


\section{User Study}
\looseness=-1
% ns3 - new version
%%%%%%%%%%%%%%%%%%%%
To best design \textsc{BIIG} to the preference of perspective users, we interviewed $5$ such potential users about their impression of current natural language (NL) insights, whether they can tolerate inaccuracies or approximations in the text, and how they use insights to build a report. All users confirmed that current template-based NL insights are often not fluent enough and can not be used as-is. Most users expressed tolerance to some inaccuracies, mainly rounding, w.r.t numerical values, and light editorial changes of cumbersome column names as long as meaning is maintained. In contrast, spurious addition of external knowledge or modifying categorical values were considered unacceptable. We considered those inputs when developing our system, and once done, recruited $3$ additional experts to provide feedback. Overall, these experts found \textsc{BIIG} intuitive and easy to use and were excited by its potential value to save time when creating insights. The option to manually edit insights seemed important, while adding context through title seemed to require some learning. They also suggested potential improvements - e.g., presenting the level of confidence of the system in the generated insights, and introducing a search box when many insights are generated - which we intend to consider in future work. 

% ns3 - prev version
%%%%%%%%%%%%%%%%%%%%%
% As mentioned above, we determined some features to be supported by \textsc{BIIG} %our system based on experience of analysts employing current Natural Language (NL) insight generators for BI. We interviewed five potential users about their impression from current NL insights, whether they can tolerate inaccuracies or approximations in the NL, and how they use NL insights while building a report. All users confirmed that current NL insights are not sufficiently fluent and often can not be used as-is. Most pronounced readiness to tolerate some inaccuracies, mainly rounding, w.r.t numerical values, and light editorial changes of long or cumbersome column names as long as semantic is maintained.
% (numbers, GPS coordinates, etc), 
% i.e., rounding numbers. 
% Also, when the name of a column or a field 
% in cases where column name 
% is long or cumbersome, they may accept some editorial changes as long as the semantic is maintained. 
% Introducing of external knowledge or modifying of categorical values, in comparison, were announced unacceptable. The generated NL insights are often presented directly from the system rather than exporting them into an external tool.
% The two main formats of working with an NL insight generator were reported to be either directly using the system during the presentation, or copying the insights along with the input chart into the generated report/slides and editing them there. 
% We considered those inputs when developing our system, and once completed,
% Once the system was ready, 
% we recruited another three experts to experience with it and to provide feedback. % that are extensively working in the domain, having more than 10 years of experience 
% provided them with the tool and asked them on their experience and feedback. 
% These experts found the system very intuitive and easy to use (adding the context seemed like a process with a learning curve), and were excited 
% and all shown excitement 
% by its usefulness w.r.t saving time when creating the insights and their quality. 
% They also liked the option to manually edit the insights. They suggested several improving features, 
% improvements 
% like presenting 
% including showing 
% the level of confidence of the system in the generated insights, and introducing a search box (mainly for 
% the use-case where there are 
% complex tables that yield a long list of insights).


==> 6_conclusions.tex <==
\section{Conclusions and Future Work}
\label{discussion}

% ns3 - new version
%%%%%%%%%%%%%%%%%%%%
\looseness=-1
\textsc{BIIG} is a system using neural models for generating insights from tables for BI analysts. 
The neural model is trained on a new large-scale dataset in the BI domain, to be released as part of this work, comprising pairs of analysis-internal-representation and insight text. While the level of factuality attained by \textsc{BIIG} exceeds previous works, a neural model is always prone to some level of errors. By facilitating editorial changes to the generated sentences, we enable users to easily correct and customize the insights. For future work, we aim to improve the the training data by better matching the intermediate representations to the insights, and to explore additional data augmentations methods, to cover a wider range of insight types. In addition, we intend to expand our user study, and further improve the system based on feedback from real world users. 
% *ns3 
% 1. When we say we outperform others - this must have some evidence mentioned earlier, perhaps when we present the res in Table 3
% 2. 
% ns3 - previous version
%%%%%%%%%%%%%%%%%%%%%%%%%
% \textsc{BIIG} is the first attempt of using neural models for generating high quality insights from tables for analysts for the BI domain. The model is trained on a new large-scale dataset from a new domain of BI that is beneficial to our research community. %, that qualifies for a commercial deployment. While notably, the level of factuality attained by \textsc{BIIG} outperforms previous works, we can not realistically expect a neural model system to generate flawless text, in particular for rigid business data. By facilitating editorial changes to the generated sentences, we enable users to easily correct and customize the insights. For future, we aim to reduce erroneous training by better matching the intermediate representation to the insights in the training dataset. In addition, we plan to improve the quality of the language model by exploring additional augmentations, and expanding over to more insight types. 

% \section{Conclusions and Future Work}
% \label{conclusion}

\section{Limitations}
% ns3 - new version
The main technical limitation of our work is related to the generative model that may inject extra words and excessive information, not present in the input. This is a well known issue with generative models. Possibly, highlight some suspicious text using various heuristics may reduce the impact of this limitation in practical use.  In addition, since the system was not yet deployed, our Recommender module is relatively simple. To improve this module we need to collect more comprehensive feedback from interactions with real world users. 
% ns3 - previous version
% The main technical limitations of our work are related to the model that at times injects extra words and excessive information, not present in its input. In addition, since the system was not yet deployed, our Recommender module is relatively simple. In order to make it better and more involved, we need to collect more feedbacks from interactions with users.


\section{Ethical considerations}
% ns3 - new version
The goal of the system is to automate insight generation. It might, therefore, potentially, take over responsibilities of experts/developers who engineer the templates in existing systems. We should note, though, that experts may still be involved in the process in new ways, such as: (a) review of (samples of) the training data; (b) collecting and exploring of editorial changes made by users via our editing feature; and more. More broadly, as any system that is based on a ML model, our system comes with all considerations that apply to the use of ML models, that require avoiding blind trust, taking into account potential bias in the training data of the system, and more. 
% ns3 - previous version
% The goal of the system is to automate text generation. It might, therefore, potentially, take over responsibilities that were until now laid upon the shoulders of analysts who authored the insights, or experts/developers who engineered the templates. We should note, though, that experts may still be involved in the process in new ways, such as: (a) review of (samples of) the training data, (b) collecting and exploring of editorial changes made by users via our special editing feature.And, generally speaking, as any system that is based on ML model, our system comes with all considerations that apply to the use of ML models, including understanding their limitations and avoiding blind trust. 



==> model_old.tex <==
\section{Methodology}
\label{methods}

\subsection{Table $\Leftrightarrow$ RDF triplets}
\subsection{RDF triplets $\Leftrightarrow$ text}

\subsection{Statista}
Statista\footnote{\url{statista.com}} is an online platform that regularly publishes and updates pages of tabular data on a vast variety of 25 general topics including economics, sports, demographics, market and opinion research, education, and more. Each webpage in the site comprises a \emph{data table} (csv), a \emph{chart} illustrating the data, and relevant \emph{topic}, \emph{title} and \emph{summary} composed by a human, expert in the field discussed. We crawled around $100K$ publicly accessible Statista webpages during December 2021. From each page, constituting as a dingle data-point, we downloaded the following instance: (data table, topic, title, summary)

\subsection{Data Creation}
In the following section, we describe creating out RDF-to-text dataset from Statista data.
We first explain how we extract (data table, candidate insight) pairs from each (data table, summary).
We then 


\subsubsection{Candidate Insight Extraction}
\label{sec:Insight-types} 
Our aim is to generate insights %(each being a single sentence) 
reflecting information observed in the data table. In the collected data, these observations are assumed to be expressed in the summary. Thus, our first step in preparing a training dataset is to extract sentences that seem to reflect insights, from the summary. 
We split each summary into sentences, then use rule-based heuristics for this identification, verifying, among other features, that the sentence contains a data table cell and its coordinates (column/row names), or a commonly verbalized alternative thereof (like number approximation, or plural/singular inflection). Inspired by industry practices\footnote{\url{docs.microsoft.com/en-us/power-bi/consumer/end-user-insight-types}} and academic works~\cite{chen2020logical,perlitzDiversity2022} we define a list of $6$ supported types including: superlative (max, min), aggregation (average, sum), comparison, trend (for time-series data), value/most recent (for time-series data), and correlation. For each type we compiled a dictionary of English words that may indicate the type and used it to detect relevant sentences. For example, for insight type ``trend'' we look for terms like: ``peak'',``grew'', ``decline'', ``decrease'', ``drop'', etc.
To evaluate the quality of the extraction, we randomly extracted $200$ sentences and their assigned types and asked 3 experts to verify the types. The quality was $91\%$. In total, for the $100K$ webpages, we extracted around $150K$ candidates of insights sentences. % each is associated with at least one type. For example, this sentence ``In 2022, the growth of China's tourism industry contribution to GDP amounted to 59.9 percent, down from 9.3 percent in the previous year.'' includes both \textit{most recent} and \textit{comparison types}.
% In parallel, we calculate per table all the relevant types. 


% of each such identified insight.

% A data table is made up of a categorical column $X$ and one or more measure columns $Y$.

% We identified several types of insights, according to the type of information they convey about the data table. This is an initial list, that can be readily expanded.

% With each type $t$, we associate (1) a computation of a value over the \emph{data table}, or a verification of a numerical property, and (2) a list of English words whose inclusion in a sentence may indicate that the sentence conveys an information of type $t$.
% \michal{Do We need this description of the calculation at all? not sure} \yotam{I don't think so...}
% For type related computation of values, insight types superlative (max, min), and aggregation (average, sum) refer to a numeric value computed, as the name suggests, over one measure column of the data table. Over such a column we can also refer to an insight of type COMPARE that compares two cells, indicating which is lower in value, and whether both cells belong to the highest values in the column, in which case the potential insight is of type FOLLOW.

% In the rather frequent case in our dataset, when a column is all dates -- typically, years, or pairs of month and year, we may also refer to the MOSTRECENT insight that conveys the value in the most recent cell of the column. In the dates case, we also have the (time-sequence) TREND\_UP or TREND\_DOWN of the values along the column.
% \michal{until here}


\subsubsection{RDF Representation}
\label{sec:RDF-creation}

We express insight and relevant context as RDF triplets, in a simple, flexible and extendable format inspired by the DART dataset~\cite{nan-etal-2021-dart}. Given the data table from Figure~\ref{fig:process-example}, Table~\ref{tab:RDF-example} shows the corresponding examples of the supported insights, and their RDF representation. For example, \texttt{[2022, MAX\_Market cap, 81.2]} expresses the fact that along the measure column named ``Market cap'', the maximum value is $81.2$, and it is obtained in $2022$. The context reflecting the title is captured by \texttt{[CONTEXT, TITLE, ``Worldwide cheese market cap'']}.  %that we adapted for our current use. 
% For example, \texttt{[2018, MAX\_Yearly sales in million dollars, 7.2]}
% % \linebreak
% % E.g.,
% % \linebreak
% % \texttt{
% % [2018, MAX Yearly sales in million dollars, 7.2]}
% % \linebreak
% expresses the fact that along the measure column named ``Yearly sales in million dollars'', the maximum value is $7.2$, and it is obtained in $2018$.
% In addition, we also associate context as an RDF triplet reflecting the title, e.g.,  
% %With each Statista case, we also associate an RDF triplet reflecting the \emph{title}. E.g.:
% %\linebreak
% \texttt{[CONTEXT, TITLE, ``Sales of cloths in California'']}
% %\linebreak

% \begin{figure}[t]
% \begin{center}
%   \includegraphics[width=1\columnwidth]{figures/RDF_example.pdf}
%  \end{center}
%   \caption{An example of a table and its RDF representation for supported insights types. \yotam{the examples here are not good, specifically: (1) what is title? (2) is previous still on?, (3) why does trend have a value triplet?}}~\label{fig:RDF-example}
% \end{figure}

\begin{table*}
\resizebox{\textwidth}{!}{
\small
\begin{tabular}{|p{3cm}|p{15cm}|}
 \hline
 Insight type  & RDF Triplets
 \\ [0.5ex] 
 \hline\hline
 Superlative (Max, Min)& \texttt{[[‘2022’, ‘MAX\_Market cap’, ‘81.2’]]} \\ 
 \hline
 Aggregation (sum, avg) & \texttt{[[‘51.38’, ‘Market cap’, ‘AVERAGE’]]}\\
 \hline
 Comparison & \texttt{[[‘2022', ‘VALUE\_Market cap', ‘81.2'], [‘2021', 'VALUE\_Market cap', ‘76.1'], [‘2021', ‘LOWER\_Market cap’, ‘2022']]} \\
 \hline
 Trend & \texttt{[[‘1960-2022', ‘TREND\_Market cap', ‘UP], [‘1960', ‘VALUE\_Market cap', ‘14.1'], [‘2022', ‘VALUE\_Market cap’, 81.2']]} \\
 \hline
 Value & \texttt{[[‘2022', ‘VALUE\_Market cap', ‘81.2']]]} \\
 \hline
 Correlation &  \\
 \hline
Title & \texttt{[[CONTEXT, TITLE, ``Worldwide cheese market cap'']
]} \\
 \hline
 \end{tabular}
 }
 \caption{Examples of RDF representations for supported insights types for the data table appears in Figure~\ref{fig:process-example}.}~\label{tab:RDF-example}
\end{table*}





\subsubsection{RDF $\Leftrightarrow$ Candidate Sentence Matching}
\label{sec:training-data-creation}

\yotam{discuss data and factuality: https://vimeo.com/385210503, table 5 dart}
Each candidate insight sentence extracted in \ref{sec:Insight-types}, includes some information, namely: \textcolor{blue}{type(s)} associated to it, \textcolor{orange}{numeric value(s)} (textual or numeric) and some \textcolor{mygreen}{column/row name(s)}. Once we extract these from the candidate, we verify that indeed the information in the candidate sentence is aligned with the the information in the data table. For example, for the given table in Figure~\ref{fig:RDF-example} and a sentence ``The \textcolor{blue}{average} number of cheese \textcolor{mygreen}{market cap} across the years \textcolor{mygreen}{1960-2020} is \textcolor{mygreen}{51.38}'', we need to verify that the average of the the market cap column is indeed around 51 and that those year range is covered by the table. 
% Given a Statista webpage, we compute, for each measure column $Y$ in the \emph{data table}, the features associated with each type $t$ above. Then, we go over the sentences of the \emph{summary}, looking for a sentence that contains the feature (i.e., a cell value and coordinates, or a commonly verbalized alternative thereof; e.g., for the above triplet, the sentence is to contain both 2018 and 7.2), and any of the dictionary words associated with $t$ ('peak', 'highest', etc. in our example).
% Note that a given sentence may satisfy the feature triplet and the dictionary words of more than one type.
Once the correctness of the candidate is verified, we add a pair of (\textit{tripletset}, sentence) to the training data.
The tripletset contains all the RDF triplets expressing computed features that matched to this sentence, along with the title triplet. For example, \{\texttt{[[‘51.38’, ‘Market cap’, ’AVERAGE’],[CONTEXT, TITLE, ``Worldwide cheese market cap 1960-2020'']]},``The average worldwide cheese market cap across the years 1960-2020 is 51.38''\}.
In addition to using this set for generation training, we also use the training set of our data to learn the frequency distribution over groups of triplets.
%, as they are grouped together into a set paired with one insight. %Note that a given sentence may satisfy more than one type.

\subsubsection{RDF-triplets Recommendation}
\label{sec:ranking}
We present two different approaches to select which insights will be presented to the user.\\
\textbf{Uniform.}
The uniform approach provides the user with all relevant insights for a given data table, each verbalized into a standalone sentence. This enables the user with an easy and flexible way to select which insights she is interested in.
\\
\textbf{Prior}. A direct outcome of our collected data is an associated distribution of the types. Specifically, we segmented the data into groups using 3 verticals: time-series (y/n), multi-column (y/n), and topic (list of 25), resulted in 100 segments. For each segment, we collect a distribution of its insights types. This segmentation allows us a more fine granular view of what other experts found interesting in each segment. Given that a data table belong to some segment, we will sample from its distribution between 4 to 6 insights.

\subsubsection{Dataset Expansion}

\begin{figure}
\begin{center}
  \includegraphics[width=1\columnwidth]{figures/trainset_type_dist.png}
 \end{center}
  \caption{\textbf{Training set type distribution}}~\label{tab:insight_dist}
\end{figure}

Our initial training set type distribution, as illustrated in Figure~\ref{tab:insight_dist} is showing a clear bias towards the simpler non aggregate types (e.g. VALUE), leaving very little examples for the more complex types (e.g. SUM, AVERAGE).
The scarcity of training example for these types prevented the model from properly generating semantically consistent texts, a major priority for our system.
To circumvent this difficulty, we propose to augment the labeled training dataset with additional noisy labeled data, comprising of RDF triplets gathered from the training set tables and corresponding text noisy labels generated by a Large Language Model (LLM).
Specifically, we generated RDF triplets corresponding all types but VALUE. Gathering this unlabeled set was done in a similar manner to the labeled set discussed in \ref{sec:training-data-creation}, differing in the RDF triplets <-> text insight matching that did not take place here.
Following the generation of the unlabeled dataset, we generated noisy labels via few-shot learning with \textit{GPT-J-6B}~\cite{gpt-j}, a 6 billion parameter, autoregressive text generation model trained on \textit{The Pile} \cite{gao2020pile}. For each unlabeled example, we pre-pended 3 (RDF triplets, text insight) example pairs obtained from the labeled training set according to its type, (an example of such input can be found in figure \ref{fig:few-shot}). Given this model input, the generated sequence was then taken as the noisy label.

\begin{figure*}[t]
\begin{center}
  \includegraphics[width=1\textwidth]{figures/few_shot.png}
 \end{center}
  \caption{\textbf{Few-shot example}}~\label{fig:few-shot}
\end{figure*}



\subsection{Model}

\begin{table*}[t]
\centering
% \resizebox{\textwidth}{!}{

\begin{tabular}{lc|cccccc}
Model      & Params & BLEU~$\uparrow$ & METEOR~$\uparrow$ & TER~$\downarrow$ & chrF++~$\uparrow$ & PARENT $\uparrow$ & BLEURT~$\uparrow$  \\ 
\hline
t5-small   & 60M    & 40.18           & 0.58              & 56.69            & 59.34             & 0.36              & 0.27               \\
t5-base    & 220M   & 47.73           & 0.64              & 50.15            & 64.60             & 0.43              & 0.35               \\
bart-base  & 140M   & 49.54           & 0.65              & 48.50            & 65.60             & 0.44              & 0.35               \\
bart-large & 400M   & 49.98           & 0.65              & 49.39            & 66.13             & 0.44              & 0.35               \\
t5-large   & 770M   & \textbf{51.52}  & \textbf{0.67}     & \textbf{47.28}   & \textbf{67.21}    & \textbf{0.46}     & \textbf{0.39}            

% \begin{tabular}{cc|ccccccc}

% Model &  Params & BLEU $\uparrow$ & METEOR $\uparrow$ & TER $\downarrow$ & chrF++ $\uparrow$& BERTScore $\uparrow$ & BLEURT $\uparrow$ & PARENT $\uparrow$ \\ \hline
% BART base  & 140M & && & &  &  &  \\ 
% BART large & 400M & && & &  &  &  \\ 
% T5 small   & 60M & & && &  &  &  \\ 
% T5 base    & 220M & & && &  &  &  \\ 
% T5 large   & 770M & & & &&  &  &  \\ 

\end{tabular}
% }
\caption{\textbf{Models results on the test set of \yotam{name dataset}}}

\end{table*}

Aiming for maximal simplicity and flexibility we followed~\cite{harkous2020have} and chose to frame RDF-to-Text as a sequence-to-sequence problem. To prevent information loss attributed to the structure of the tripleset we encode this structure in to the linerized representation by replaceing the \texttt{","} separators appearing inside and between  triples with \texttt{[W]} and \texttt{[B]} tokens respectively, these were then were defined as new special tokens for the model to learn.
we used two Pre-trained Language model (PLM) families, T5~\cite{raffel2020exploring} and BART~\cite{lewis2019bart}, both are based on the Transformer \textit{encoder-decider} architecture~\cite{vaswani2017attention} and mostly differ in their pre-training corpus and pre-training scheme. following~\cite{ribeiro2020investigating}, we specifically experimented with with \textit{t5-small} / \textit{t5-base} / \textit{t5-large} (60M / 220M / 770M parameters) and \textit{bart-base} / \textit{bart-large} (140M / 400M parameters) as available in the \textit{huggingface-hub}\footnote{\url{https://huggingface.co/models}}.

\subsubsection{RDF-to-Text Evaluation}

We use a wide range of automatic metrics to evaluate the text generation quality.
We report the official WebNLG~\cite{webnlg-2017} evaluation metrics BELU~\cite{papineni2002bleu}, METEOR~\cite{banarjee2005meteor} and TER~\cite{snover-etal-2006-ter}, along with chrF++~\cite{popovic-2017-chrf}, a character n-gram based metric.
Since the above n-grame based metrics are limited in their capacity to consider the semantic meaning of words \cite{novikova-etal-2017-need}, we additionally report BLEURT~\cite{bleurt}, that had been shown to be a top performer along the learned semantic similarity metrics. To also account for generation consistency between the RDF triplet and text, we also include PARENT~\cite{dhingra2019parent}, which aligns reference, generated text and  triplet n-grams.

\subsubsection{Implementation Details}
All models were fine-tuned for 10 epochs and a batch size of $64$ (the maximum batch size that fits our largest model on our GPU). We used the \textit{adafactor} optimizer~\cite{shazeer2018adafactor}, with the default learning rate of $1\times10^{-4}$ and the common autoregressive cross entropy loss. Input and output sequence length were set to 64 tokens of the default models tokenizers.
A single NVIDIA A100 GPU was used for fine-tuning. All our pretrained models where taken from the \textit{huggingface-hub}\footnote{\url{https://huggingface.co/models}}. Our Implementation is based on Huggingface Transformers~\cite{wolf2019huggingface} version 4.20.1 and pytorch~\cite{paszke2019pytorch} version 1.9.0.

\section{Generation}
\label{sec:generation}


% We randomly select a group $G$ of types, according to the prior learned in the training stage. We then realize $G$ as a set of triplets, by computing the implied features over the measures, and feed into the model which generates an insight therefrom. 



==> tool.tex <==
\usepackage{todonotes} % for comments

\newcommand\BibTeX{B\textsc{ib}\TeX}
\newcommand{\RomanNumeralCaps}[1]{\MakeUppercase{\romannumeral #1}}
\makeatletter
\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
\makeatother

\makeatletter
\newcommand{\printfnsymbol}[1]{%
  \textsuperscript{\@fnsymbol{#1}}%
}
\makeatother

\newcommand{\liat}[1]{\textcolor{orange}{L: #1}}
\newcommand{\noam}[1]{\textcolor{purple}{N: #1}}
\newcommand{\dafna}[1]{\textcolor{red}{D: #1}}
\newcommand{\michal}[1]{\textcolor{brown}{M: #1}}
\newcommand{\yotam}[1]{\textcolor{blue}{Y: #1}}
\newcommand{\eyal}[1]{\textcolor{cyan}{E: #1}}

